Analysis of Distributed Ledger Technologies for Industrial Manufacturing

In recent years, industrial manufacturing has undergone massive technological changes that embrace digitalization and automation towards the vision of intelligent manufacturing plants. With the aim of maximizing efficiency and profitability in production, an important goal is to enable flexible manufacturing, both, for the customer (desiring more individualized products) and for the manufacturer (to adjust to market demands). Manufacturing-as-a-service can support this through manufacturing plants that are used by different tenants who utilize the machines in the plant, which are offered by different providers. To enable such pay-per-use business models, Distributed Ledger Technology (DLT) is a viable option to establish decentralized trust and traceability. Thus, in this paper, we study potential DLT technologies for an efficient and intelligent integration of DLT-based solutions in manufacturing environments. We propose a general framework to adapt DLT in manufacturing, then we introduce the use case of shared manufacturing, which we utilize to study the communication and computation efficiency of selected DLTs in resource-constrained wireless IoT networks.

==> package.tex <==
\usepackage{times}
\usepackage{amsmath,epsfig}
\usepackage{amssymb}
\usepackage{amsfonts}
\usepackage{array,dcolumn}
\usepackage[ruled,vlined,linesnumbered]{algorithm2e}
\usepackage{subcaption}
\usepackage{psfrag}
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{balance}
\usepackage{accents}
\usepackage{booktabs, adjustbox}
\usepackage{cite}
\usepackage[all]{xy}
\interdisplaylinepenalty=2500
\usepackage{dsfont}
\usepackage{hyperref}
\usepackage{url}
\usepackage{xcolor}
\usepackage[nolist]{acronym}
\usepackage{graphicx}
\usepackage{float}
\usepackage{threeparttable}
\usepackage{cancel}
\usepackage[official]{eurosym}
\usepackage{chemformula}
\usepackage{subcaption}
\usepackage{graphicx}
\usepackage[utf8]{inputenc}
\usepackage[english]{babel}
\usepackage{filecontents, pgffor}
\usepackage{listings, xcolor}
\usepackage{xcolor}
\usepackage[linesnumbered,ruled,vlined]{algorithm2e}
\usepackage{mathtools,amssymb,lipsum, nccmath}
\usepackage{cuted}
\usepackage[normalem]{ulem}
\usepackage{chemformula}
%\usepackage{minted}



\def\undb#1{\mbox{\bf{#1}}}

%\include{pythonlisting}
\def\BibTeX{{\rm B\kern-.05em{\sc i\kern-.025em b}\kern-.08em
    T\kern-.1667em\lower.7ex\hbox{E}\kern-.125emX}}

\newcommand\mycommfont[1]{\footnotesize\ttfamily\textcolor{blue}{#1}}
\SetCommentSty{mycommfont}

\DeclareMathOperator*{\argminA}{arg\,min}

\hypersetup{
     colorlinks = true,
     linkcolor = blue,
     anchorcolor = black,
     citecolor = blue,
     filecolor = blue,
     urlcolor = blue
     }

\hyphenation{op-tical net-works semi-conduc-tor}


==> table-co2.tex <==

\begin{table} [h!]
\centering
\caption{Carbon FootPrint of private DLT testbed with 5 \emph{DLTs} calculuated in Germany market running per hour }
\begin{tabular}{p{1.7cm}||p{1.5cm}|p{2cm}|p{2cm}|p{2cm}|p{2cm}|p{2cm}}
\toprule
\textbf{Platform}  & \textbf{Power of Machine (kW)} & \textbf{Energy consumed on Average (kWh)} &  \textbf{Avg. CPU Usage for Blockchain Operation (\%)} & \textbf{Energy Consumed for Blockchain operation (kWh)} & \textbf{Greenhouse gas (GHG) emission in DE (kg \ch{CO2}-eq/kWh)}** & \textbf{GHG emission per blockchain operation (kg \ch{CO2}-eq)} \\
\midrule
\textit{Hyper.Fabric}        & 0.06  & 0.06 & 0.625\% & 375 $\cdot 10^{-6}$     & 0.540 & 203 $\cdot 10^{-6}$ \\
\textit{Ethereum }          & 0.06  & 0.06 & 82.35\% & 49392 $\cdot 10^{-6}$    & 0.540 & 26682 $\cdot 10^{-6}$  \\
\textit{Quorum}             & 0.06  & 0.06 & 0.65\% & 390 $\cdot 10^{-6}$       & 0.540 & 211 $\cdot 10^{-6}$ \\
\textit{IOTA}               & 0.06  & 0.06 & 0.61\% & 366 $\cdot 10^{-6}$       & 0.540 & 198 $\cdot 10^{-6}$ \\
\textit{Solana}             & 0.06  & 0.06 & 0.61\% & 366 $\cdot 10^{-6}$       & 0.540 & 198 $\cdot 10^{-6}$  \\
\bottomrule
\end{tabular}
%\begin{tablenotes}
%\centering
%      \small
%      \item *The Electronic Cost of \emph{DLT} nodes is computed using the PowerTop\cite{powertop71:online}
      %\item **Greenhouse gas (GHG) emission intensity of the Germany energy grid (kg CO2-eq /kWh)
%    \end{tablenotes}
\label{tab:co2}
\end{table}


==> table-comparison.tex <==

\begin{table}[t!]
\centering
\caption{Comparison of different enterprise DLT platforms}
\label{tab:comparison}
\begin{tabular}{ p{2.3cm} ||p{2.5cm} p{2.5cm} p{2.7cm}  p{2.5cm} p{2.5cm}}
\toprule
& \textbf{Hyper. Fabric} \cite{androulaki2018hyperledger}   & \textbf{Quorum} \cite{baliga2018performance}      & \textbf{Ethereum} \cite{vujivcic2018blockchain}  & \textbf{IOTA} \cite{popov2019iota} & \textbf{Solana}\cite{yakovenko2018solana} \\ 

\midrule
%                                Fabric              Quorum                 Ethereum            IOTA                  Solana
\textit{DLT type}                & Private           & Private              & Public / Private  &  Public / Private   &  Public / Private   \\ 
\textit{Goals}                   & Open DLT framework & Open, based on Ethereum & Broad ecosystem   & Lightweight &  High scalability      \\
\textit{Application}             & Enterprise DLT    & Enterprise DLT       & DApps             &  IoT                &  DApps     \\ 
\textit{Governance}              & Linux Foundation  & ConsenSys            & ETH Foundation    &  IOTA Foundation    &  Solana   \\
\textit{Cryptocurrency}          & N/A                & N/A                  & Ether (ETH)       &  MIOTA              &  SOL            \\
\textit{Consensus}               & Pluggable         & Voting Protocol      & PoW               &  Tangle             &  PoH          \\
\textit{Smart Contract}          & nodejs, go, java  & Solidity             & Solidity    &   {Solidity, Go, Rust}        &  Rust    \\
\textit{Throughput}              & $\sim$2000 tps    & $\sim$100 tps        & $\sim$100 tps     &  1000$\sim$1500 tps &  $\sim$1400 tps     \\
\textit{Latency}   & $\sim$250 ms      & $\sim$414 ms           & $\sim$2150 ms        & $\sim$ 258 ms           & $\sim$ 500 ms      \\
\bottomrule
\end{tabular}
\end{table}
